Hall-Littlewood polynomials, boundaries, and $p$-adic random matrices

We prove that the boundary of the Hall-Littlewood $t$-deformation of the Gelfand-Tsetlin graph is parametrized by infinite integer signatures, extending results of Gorin and Cuenca on boundaries of related deformed Gelfand-Tsetlin graphs. In the special case when $1/t$ is a prime $p$ we use this to recover results of Bufetov-Qiu and Assiotis on infinite $p$-adic random matrices, placing them in the general context of branching graphs derived from symmetric functions. Our methods rely on explicit formulas for certain skew Hall-Littlewood polynomials. As a separate corollary to these, we obtain a simple expression for the joint distribution of the cokernels of products $A_1, A_2A_1, A_3A_2A_1,\ldots$ of independent Haar-distributed matrices $A_i$ over the $p$-adic integers $\mathbb{Z}_p$. This expression generalizes the explicit formula for the classical Cohen-Lenstra measure on abelian $p$-groups.

==> preamble.tex <==
%note: I commented out most packages to avoid conflict issues with the oupau template, but otherwise this agrees with usual preamble
%\usepackage{anysize}
%\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{amsmath,amscd}
%\usepackage[utf8]{inputenc}
%\usepackage[foot]{amsaddr}
%\begin{CD}
%A @>a>> B\\
%@VVbV @VVcV\\
%C @>d>> D
%\end{CD}
\usepackage{amssymb}
\usepackage{stmaryrd}
\usepackage{wasysym}
\usepackage{mathrsfs}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{enumitem}
%\usepackage{epstopdf}
\usepackage{dsfont}
\usepackage{soul}
\usepackage{filecontents}
\hypersetup{colorlinks=true,linkcolor=black,citecolor=black}
\usepackage{color}
\usepackage[all]{xy}
\usepackage{float}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{setspace}
\usepackage{comment}
\usepackage{tikz}
\usepackage{mathdots}
%\usepackage[myheadings]{fullpage}

\bibpunct{[}{]}{,}{n}{,}{;}
%this is courtesy of https://tex.stackexchange.com/questions/241509/natbib-error-with-journal-of-complex-networks-oup, stops latex from taking issue with alpha citation styles

\setcounter{tocdepth}{1} %makes table of contents not include subsections
\numberwithin{equation}{section}
\parskip=0.05in 
\parindent=0.23in
%\pagestyle{plain}
%\newcommand\mtop{1in}
%\newcommand\mbottom{1in}
%\newcommand\mleft{1in}
%\newcommand\mright{1in}
%\usepackage[top = \mtop, bottom = \mbottom, left = \mleft, right=\mright]{geometry}
\newtheorem{name}{Printed output}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{example}[thm]{Example}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{claim}[thm]{Claim}
\newtheorem{lem}[thm]{Lemma}
%\newtheorem{problem}[1]{\textbf{Problem #1}}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\theoremstyle{definition}
\newtheorem{defi}{Definition}
\newtheorem{notation}{Notation}
\newtheorem{rmk}{Remark}
\newcommand*{\problem}[1]{\textbf{Problem #1}}
%\newcommand*{\exercise}[1]{\textbf{Exercise #1}}
%\usepackage{scalerel,stackengine}
%\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
    {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
  }{\textheight}% 
}{0.5ex}}%
\stackon[1pt]{#1}{\tmpbox}%
}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}

%makes table of contents indent properly, taken from https://tex.stackexchange.com/questions/51760/table-of-contents-with-indents-and-dots
\begin{comment}
\makeatletter
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima
      \ifcase #1
       \or\or \hskip 1em \or \hskip 2em \else \hskip 3em \fi%
      #6\nobreak\relax
    \hfill\hbox to\@pnumwidth{\@tocpagenum{#7}}\par% <---- \dotfill -> \hfill
    \nobreak
    \endgroup
  \fi}
\makeatother
\end{comment}

%Steve Miller's fix commands
\newcommand{\todo}[1]{\textcolor{red}{\textbf{(#1)}}}
\newcommand{\fix}[1]{\textcolor{red}{\textbf{\large (#1)\normalsize}}}
\newcommand{\fixed}[1]{\textcolor{green}{~\\ \textbf{\large #1\normalsize}}\\}

%symbols
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\bbM}{\mathbb{M}}
%\renewcommand{\H}{\mathbb{H}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\X}{\mathcal{X}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mc}{\mathcal}
\renewcommand{\sl}{\mathfrak{sl}}
\renewcommand{\sp}{\mathfrak{sp}}
\newcommand{\gl}{\mathfrak{gl}}
\renewcommand{\o}{\mathfrak{o}}
\newcommand{\g}{\mathfrak{g}}
\newcommand{\bbone}{\mathbbold{1}}
%\renewcommand{\l}{\lambda}
\newcommand{\eps}{\epsilon}
\renewcommand{\Re}[1]{\text{Re}(#1)}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\text{Im}}
\newcommand{\cov}{\text{Cov}}
\newcommand{\var}{\text{Var}}
\newcommand{\pfrac}[2]{\left(\frac{#1}{#2}\right)} 
\newcommand{\bfrac}[2]{\left[\frac{#1}{#2}\right]}
\renewcommand{\cfrac}[2]{\left\{\frac{#1}{#2}\right\}}
\newcommand{\liminfty}{\lim_{n\rightarrow \infty}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\dde}[3]{\left. \frac{d #1}{d #2} \right|_{#3}} %derivative evaluated at something
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dderiv}[2]{\frac{d #1}{d #2}}
\newcommand{\curleps}{\mathcal{E}}
\newcommand{\op}{\oplus}
\newcommand{\ot}{\otimes}
\newcommand{\mm}{\mathfrak{m}}
\newcommand{\ma}{\mathfrak{a}}
\newcommand{\mb}{\mathfrak{b}}
\newcommand{\mg}{\mathfrak{g}}
\newcommand{\mn}{\mathfrak{n}}
\newcommand{\mh}{\mathfrak{h}}
\newcommand{\hmn}{\hat{\mathfrak{n}}}
\newcommand{\hmg}{\hat{\mathfrak{g}}}
\newcommand{\hmh}{\hat{\mathfrak{h}}}
\newcommand{\tmu}{\tilde{\mu}} 
\newcommand{\tz}{{\tilde{z}}}
\newcommand{\tw}{{\tilde{w}}}
\newcommand{\hsl}{\widehat{\mathfrak{sl_2}}}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\dla}{\langle \langle}
\newcommand{\dra}{\rangle \rangle}
\newcommand{\inj}{\hookrightarrow}
\newcommand{\tth}{^{th}} 
\newcommand{\px}[1]{\pd{}{x_{#1}}}
\newcommand{\py}[1]{\pd{}{y_{#1}}}
\newcommand{\chr}[3]{\Gamma_{#1 #2}^{#3}}
\newcommand{\bX}{\bar{X}}
\newcommand{\bY}{\bar{Y}}
\newcommand{\bZ}{\bar{Z}}
\newcommand{\na}{\nabla}
%random commands used in p-adic RMT paper which should probably get removed in subsequent iterations of this template
\newcommand{\cv}{\check{v}}
\newcommand{\hv}{\hat{v}}
\newcommand{\tnu}{\tilde{\nu}}
\newcommand{\M}{\mu_{Haar}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hc}{\hat{c}}
\newcommand{\tkappa}{\tilde{\kappa}}
\newcommand{\tl}{\tilde{\lambda}}
\newcommand{\tm}{\tilde{\mu}} 
\newcommand{\tk}{\tilde{\kappa}} 
\newcommand{\tc}{\tilde{c}} 
\newcommand{\bl}{{\bar{\lambda}}}
\renewcommand{\bm}{{\bar{\mu}}}
\newcommand{\bk}{{\bar{\kappa}}}
\renewcommand{\hl}{{\hat{\lambda}}}
\renewcommand{\hm}{{\hat{\mu}}}
\newcommand{\hk}{{\hat{\kappa}}}
\renewcommand{\L}{\Lambda}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\tT}{\tilde{T}}
\newcommand{\G}{\mathscr{G}_t}
\newcommand{\bG}{\overline{\mathscr{G}_t}}
\newcommand{\GG}{\widetilde{\mathscr{G}_t}}
\newcommand{\K}{K}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\cP}{\mathbb{Y}}
\newcommand{\hx}{\hat{x}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\barv}{\bar{v}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tA}{\tilde{A}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\EM}{E}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\bsomega}{\boldsymbol{\omega}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\DeclareMathOperator{\Geom}{Geom}
\DeclareMathOperator{\Sym}{Sym}
%end of weird random commands
\DeclareMathOperator{\len}{len}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\rec}{rec}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\U}{U}
\DeclareMathOperator{\SU}{SU}
\DeclareMathOperator{\Vir}{Vir}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\Sig}{\mathbb{GT}}
\DeclareMathOperator{\bSig}{\overline{\mathbb{GT}}}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\GT}{GT}
\DeclareMathOperator{\tPr}{\tilde{Pr}}
\DeclareMathOperator{\tM}{\tilde{M}}
%\DeclareMathOperator{\tE}{\tilde{E}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\SN}{SN}
\DeclareMathOperator{\ESN}{ESN}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Mat}{Mat}
\newcommand{\gap}{\operatorname{gap}}
\newcommand{\sqbinom}[2]{\begin{bmatrix}#1\\ #2\end{bmatrix}}
\newcommand{\qhyp}{\;_4 \bar{\phi}_3}
\newcommand{\qhypl}{\;_2 \bar{\phi}_1}
\newcommand{\qhypm}{\;_3 \bar{\phi}_2}
\newcommand{\teps}{\tilde{\epsilon}}


%\renewcommand{\S}{\operatorname{S}}
